Narrative Transitions in Data Videos

Transitions are widely used in data videos to seamlessly connect data-driven charts or connect visualizations and non-data-driven motion graphics. To inform the transition designs in data videos, we conduct a content analysis based on more than 3500 clips extracted from 284 data videos. We annotate visualization types and transition designs on these segments, and examine how these transitions help make connections between contexts. We propose a taxonomy of transitions in data videos, where two transition categories are defined in building fluent narratives by using visual variables.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> texfiles/discussion.tex <==
\section{Design Suggestions} \label{section:discussion-design-suggestions}

Informed by the content analysis and taxonomy, we summarize a series of design suggestions for transition designs in data videos from the following three aspects, \textit{i.e.}, clip forms, content relation, and visualization types.
Given that transitions of the \textit{Refresh}, \textit{Halftime}, \textit{Camera Motion} category are not specialized for any specific content, including clip forms, content relation, and visualization types, we summarized available transitions of \textit{Preserving Guide} and \textit{Narrative Agent} in these three aspects in \autoref{fig:suggestions}.
The table presents available transition choices in different situations but with no effectiveness evaluation yet.
We take typical transitions as examples to explain our design suggestions.

\begin{figure*}[htb]
\centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
\includegraphics[width=\textwidth]{statistics-transitions.pdf}
\caption{
    (a) Five transition categories loosely ordered by the relevance of data content between scenes.
    % The martini glass shows the space of using scenarios for these transitions.
    (b) Result of our content analysis showing the statistics of visualization-to-visualization, visualization-to-non-visualization, non-visualization-to-visualization transitions in our collected videos. 
}
\label{fig:statistics-transitions}
\end{figure*}

\subsection{Clip Form}
A data video has a series of clips, some of which are data clips, while others are not.
These clips have different forms, indicating that they have different styles in presenting video content.
For example, videos such as \textit{We're quitting smoking, so why is big tobacco booming?}\cite{Guardian2019} from \textit{The Guardian}, introduce social topics through an arranged multimedia sequence, which includes expert interviewing scenes and data visualizations.
By contrast, videos, such as \textit{Global Wealth Inequality}~\cite{TheRulesOrg2013} shown in \autoref{fig:case-1}, mainly consist of animated graphics.
Some videos, such as the famous \textit{Hans Rosling's 200 Countries, 200 Years, 4 Minutes -- The Joy of Stats}~\cite{BBC2010}, are a mixture of animated data visualizations and shot scenes of the interpreter.
The transition designs in different clip forms vary.

% \textbf{Only Visualization Content}:
\textbf{Use shared visual variables to articulate the transitions between visualizations.}
Videos that have transition clips of only visualization contexts take a big proportion of 94\% (267/285) in our data video dataset.
Transitions between these clips are used to transform video content between different charts.
Staged animation in Heer and Robertson's work\cite{Heer2007} is suitable in this scenario.
In our taxonomy, this type of staged animation belongs to \textit{Preserving Guide} and \textit{Narrative Agent}.
Within these two transitions, those preserved visual variables encode the same narrative meanings of charts in the previous and coming scenes, thereby keeping the viewers oriented during the change of video context.
Transition designs between different visualizations can use \textit{RST Guide}, \textit{Staying Guide}, \textit{Updating Content}, etc., according to the forms of visualizations.
Suggestions on transitions between specific visualization types are discussed in detail in \autoref{section:discussion-vistype}.

% \textbf{Visualizations and Animated Icons}:
% \textbf{Integrate transitions with icon animations.}
\textbf{Build the connection between visualization and other video content through transitions.}
% Videos that have transition clips of visualizations and animated icons take a proportion of 79\% (226/285) in our data video dataset.
% Animations of icons (including characters) can be integrated with the animation of \textit{RST Guide} in transitions (see as \autoref{fig:intro-example}).
The transitions of \textit{Preserving Guide} and \textit{Narrative Agent} can fluently connect visualization contents with others in data videos (see as \autoref{fig:intro-example}(a)).
The transition designs of these clip forms can utilize the similar visual variables between animated icons and items of visualizations (e.g., the circular shape of icons and pie charts and the color of icons and specific encoding in charts).
These same or similar visual variables can create a bridge of non-data-driven animated icons and data-driven visualization items with a seamless meaning transformation between them.
Moreover, texts and numbers can be reused in the coming scenes as titles or labels of charts without an additional set-up animation (\autoref{fig:teaser}(a1-a3)).
% These designs also work on data videos that are in the form of stop motion animation (e.g., clips of paper cuttings or hand-drawing pictures).

% \textbf{Visualizations and Photography}:
% A mixture of photography scenes and animated visualizations present a larger amount of information than presenting every single one of them.
% Photography scenes offer viewers intuitive stimulation, while data facts of visualizations provide convincing arguments.
% The photography scenes include an expert interviewing shot scenes, reporter's monologue or static images, etc.
% There are 21\% (61/285) videos in our dataset, which have transition clips of visualizations and photography.
% Visualizations can be presented by being overlaid on these realistic scenes or being the main contents of a new scene.
% The \textit{Refresh} transition can be used in this scenario because the style of animated visualizations and shot clips are different.
% However, if visualizations are presented by real things in photography scenes (e.g., building blocks), then video designers can also use \textit{Updating Content} to show the changing process of data, such as what the video \textit{Is America Dreaming?: Understanding Social Mobility}~\cite{Brooking2014} does.
% \textit{Rack Focus} can be used to distinguish the following content from the previous one and keep viewers' attention in the new part.
% This kind of transition is used when first presenting a realistic scene, and then a visualization overlaid on it.
% \textit{RST Guide} transition can also be used in this clip form.
% The visualization and the realistic scene can be the moving guide when you opt to take apart the scene and present them on each side of it.
% In some situations, the interpreter has no interactions with contents in the scene, so the transition design mainly depends on other contents.

% Lastly, \textit{Refresh} and \textit{Halftime} can be used in all above scenarios (only visualization content, visualizations \& animated icons, visualization \& photography).
% We suspect that there are two reasons.
% First, suitable arrangements of \textit{Refresh} transitions, like \textit{Hard Cut}, can consist of continuity editing, which is a transition guidance in narrative visualizations\cite{Segel2010}.
% Second, extra designs about the \textit{Halftime} scenes or the \textit{Wipe} masks, like described in \cite{Xia2018}, allow the halftime scenes or the masks to be part of video content.

\begin{figure*}[htb]
\centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
\includegraphics[width=0.88\textwidth]{suggestions.pdf}
\caption{
    Available transitions in clip forms, content relations and visualization types.
}
\label{fig:suggestions}
\end{figure*}

\subsection{Content Relation}
Data videos are author-driven stories\cite{Segel2010}.
These videos have linear storylines presented in an arranged order of scenes.
That is, authors need to carefully consider the relationship between consecutive scenes and use elaborate transitions. 
Based on our analysis, the specific transitions can help reveal the following content relations in data videos.

\textbf{Question \& Answer}:
\textbf{Reuse elements in question when answering.}
To lead viewers from the establisher and initial parts of a story to its peak gradually \cite{Amini2015}, designers can use attractive questions as a start and then use visualizations to answer the question by presenting data facts.
In this process, the contents of the questioning scene, such as texts, icons, or even question marks, can be used to create a \textit{Preserving Guide} transition.
For example, texts of the question can be used as an \textit{RST Guide}, and they can move to the visualization as a related annotation of charts.
By doing so, the question and related answers become a fluent sequence without an abrupt change.

\textbf{Whole and Part}:
\textbf{Group items, expand colors, or zoom.}
This content relation means presenting different granularities of data in contexts.
% No strict order is imposed regarding who should be presented first when showing a relation between the whole and the part in our statistics.
By grouping partial items together or splitting them, a \textit{Merging/Splitting} transition can reveal the affiliation of partial items and the whole entity (\autoref{fig:case-1}(c1-c5), (a1-a5)).
This content relation also includes topics and subtopics.
If related contents of subtopics exist in the scene of the whole topic, then designers can use \textit{Zooming} (\autoref{fig:teaser}(d1-e1)) or \textit{Expanding Guide} (\autoref{fig:teaser}(f1-f3)) to demonstrate the subtopics in detail after the presentation of the whole topic.
Those related contents (e.g., the red point in \autoref{fig:teaser}(d1), the blue sector in \autoref{fig:teaser}(f1)) are the medium of these types of transitions.
With a zoom-in camera motion or a background expanding animation, the meaning of a further introduction of this topic can be illustrated, especially the subtopic that the expanding color or the zooming focus represents.

\textbf{Progress} and \textbf{Supplement}:
\textbf{Present items one by one.}
Telling the story progressively is common in storytelling.
If contents are planned on a canvas layout, then designers can use a \textit{Pedestal/Truck} camera motion to present them individually (\autoref{fig:case-2}(b1-b5)).
If the canvas layout is not created for scenes, then designers can use \textit{Rack Focus} to blur the previous content and present the supplement overlaid on the blurred background (\autoref{fig:teaser}(l1-l3)).
The contents of the previous scene can be an \textit{RST Guide} to conduct a supplement in the coming scenes (\autoref{fig:case-2}(c1-c5, c5-c6))
The \textit{Morphing} transition can also be used in a progress narrative to present a changing process of contents (\autoref{fig:case-3}(c1-c5)).

\textbf{Contrast}:
\textbf{Preserve contexts for comparison.}
Contrasts among different data can play a role in strong arguments for narrative.
A contrast can be gradually created.
Accordingly, visualizations in the previous scenes can be regarded as a whole \textit{RST Guide}.
The whole part translates to a new position but is preserved in the scene while making space for other contents for contrast.
For example, a designer wants to present two pie charts about the sex ratio of two classes for contrast.
After presenting the pie chart of class A, she preserves the chart and lays it on the left side of the screen.
Then, she presents the pie chart of class B on the right side.
Moreover, designers can use \textit{Narrative Agent} transitions (e.g., \textit{Scaling}) to present the contrast of data in different situations by updating related video contents (\autoref{fig:case-1}(d1-d5)).

\subsection{Data Visualization Type} \label{section:discussion-vistype}
Our content analysis demonstrates design tactics for different visualization types.
We summarize these tactics on the basis of our data video dataset and taxonomy, including how to transform \textit{from} and \textit{to} them.
The frequency of transitions \textit{from} and \textit{to} specific visualizations are presented in our supplemental materials.
% Some transition designs are not shown in our collected videos but can be inspired by the taxonomy.

We first present the general transition designs for visualizations and then specific tactics for different visualization types orderly in the following. 
If details in the visualization will be presented, then designers can use \textit{Camera Motions}, such as \textit{Pedestal/Truck} and \textit{Zooming}, to present them for demonstration.
Another way is to use \textit{Updating Content} to present these details in an arranged order.
\textit{Updating Content} can be used for presenting the update of data on the basis of the same form of charts.

Designers can make good use of the same elements in different scenes.
For example, the same color area can be used as an \textit{Expanding Guide}.
The annotation texts or icons can be used as a \textit{RST Guide}, and the same basic geometry shapes, such as circle and rectangle, can be used as \textit{Staying Guide}.

The individual visualization types have different visual components.
Accordingly, the transition designs of the varying visualization types are also distinguished according to these components.
We list the specific tactics for the following visualization types as a supplement for the general tactics mentioned above.
These types of visualization are commonly used in our data video dataset.

\textbf{Line Chart}, \textbf{Scatter Plot}, and \textbf{Bar Chart}:
These three types of charts have many necessary components, for example, axes, legends, label texts, as well as data-encoded lines, points, and bars.
Designers can take these components as a medium for the \textit{RST Guide} transition.
Besides, the axial component can also be a \textit{Staying Guide} when continuously presenting these three types of charts with different contents.

\textbf{Map}:
Maps can present spatial data.
The overview and detailed conditions of maps are essential for presenting data patterns.
\textit{Camera Motion} is a widely used transition to transform between different presenting levels or places on maps.
\textit{Zooming} can indicate the geographical information.
For instance, a particular condition of the city in a country can be shown by zooming from the whole map of the country into the city, and vice versa.
The horizontal or vertical movement of the camera, for example, \textit{Pedestal/Truck}, creates a feeling of space of the scene and reveals the relative localization of different regions.
The shape of a specific region on maps is a good choice for a \textit{RST Guide} if it is also shown in near scenes.
The color of one sub-region can be an \textit{Expanding Guide}, that is, expanded as a background color when presenting detailed data of this subregion.

\textbf{Proportional Area Chart}, \textbf{Pie Chart}, and \textbf{Donut Chart}:
These types of charts present the proportional relation of data.
The \textit{Merging} transition can gather parts that represent different categories of data from the previous scenes and combine them as a whole chart.
The \textit{Splitting} transition is on the opposite.
Varying colors are used to encode different proportional areas in these charts.
These areas can be well used to present the whole and part levels of information as the medium for the \textit{Expanding Guide} (\autoref{fig:case-3}(a1-a5)).
Designers can also use \textit{Scaling} and \textit{Morphing} transitions to present the change of proportional relation of data by revising the size or shape of changing parts.

\textbf{Diagram}:
Diagrams can present pipelines.
In contrast with statistical charts, this type of visualization presents the progress of a topic rather than the data values.
Designers can present each procedure through \textit{Pedestal/Truck} in sequence and use \textit{Zooming} to show the whole diagram at last.
The arrows between procedures can be used as the attention cues of the \textit{RST Guide} transition and link up the whole pipeline.
As for transforming from and to diagrams, icons, and texts in the procedure of a diagram can be used as the \textit{RST Guide}.

\textbf{Pictograph} and \textbf{Number, Icon and Text}:
These types of visualizations mainly consist of animated icons.
Such icons may have their animations or interactions with other elements in the scene.
Transitions from and to these visualizations can make good use of these icons, for example, taking them as the medium of the \textit{RST Guide} transition.
In that way, the rotating, scaling, and translating animations of icons are equal to the transition of scenes, thereby making the transformation seamless in the narrative.


==> texfiles/usecase.tex <==
\section{Use Case}
In this section, we demonstrate a use case (\autoref{fig:teaser}) on how to leverage our taxonomy to design a data video. 
The video is about COVID-19, which introduces the severe condition of the COVID-19 spreading by presenting a series of data facts with elaborate transitions. 
The data is collected from the official notification, and the whole video can be found in the supplementary materials. 

% First, the video designer use a series of texts as the establisher part, which indicates that this video is about the COVID-19 outbreak.
% He wants to show the data of COVID-19 cases over the world by time.
First, the video begins with a series of texts that indicate that the video is about the COVID-19 outbreak (\autoref{fig:teaser}(a1)).
With the texts preserving the keywords, a \textit{RST Guide} transition connects the previous scene with a world map to show the data of the total cases in different regions over the world (\autoref{fig:teaser}(a2-a3)).
The color depth on the map represents the severity of the infection in the corresponding area, which becomes deeper over time in China.
A \textit{Zooming} transition brings the viewer into a detailed portrait of the total confirmed case data in China (\autoref{fig:teaser}(b1-b3)).
The number rapidly increases over time.
Then, texts of date and number serve as the medium of the \textit{RST Guide} transition (\autoref{fig:teaser}(c1)).
In combination with the transition, the number seamlessly transforms into one point of the line chart (\autoref{fig:teaser}(c2-d1)).
The line steeply grows, and a \textit{Zooming} transition enlarges the presentation of the highest points of the line chart (\autoref{fig:teaser}(d1-e1)).
Then, the time stops growing, and the \textit{Updating Content} transition is used to show the details of February 12 (\autoref{fig:teaser}(e1-e2)).
The point that represents the total cases on February 12 keeps its circular shape and transforms into a pie chart of the proportion of confirmed cases in Wuhan and other places in China (\autoref{fig:teaser}(e1)).
The proportion of total confirmed cases in Wuhan is over  half of the total cases in China.
To show a further detail, an \textit{Expanding Guide} transition expands the color of the sector that represents Wuhan in the pie chart to the background of the scene, thereby indicating that the following scene is about the detailed condition of Wuhan (\autoref{fig:teaser}(f1-f3)).
A group of people icons represents the whole crowd of confirmed cases in Wuhan  (\autoref{fig:teaser}(g1)).
The icons consist of a proportional pictograph by \textit{Splitting} into three groups to show the number of existing confirmed, cured, and dead cases (\autoref{fig:teaser}(g1-g3)).
Thereafter, the icons of each group are \textit{Merged} into a proportional area chart that represents the percentage of each group (\autoref{fig:teaser}(h1-i1)).
Then, a \textit{Shrinking Guide} transition transforms the proportional area chart into the previous pie chart (\autoref{fig:teaser}(i1-i2)).
Then a \textit{Zooming} transition guide viewers' sight to the world map and raises the statistical map of total cases over the world (\autoref{fig:teaser}(j1-j2)).
As time goes, by the \textit{Updating Content} transition, the global situation turned terrible (\autoref{fig:teaser}(k1-k3)).
Lastly, a \textit{Rack Focus} transition blurs the world map and shows a proposal that the whole world should unite together to defeat COVID-19 (\autoref{fig:teaser}(l1-l3)).
